One-way Communication Complexity of Minimum Vertex Cover in General Graphs

We study the communication complexity of the Minimum Vertex Cover (MVC) problem on general graphs within the \(k\)-party one-way communication model. Edges of an arbitrary \(n\)-vertex graph are distributed among \(k\) parties. The objective is for the parties to collectively find a small vertex cover of the graph while adhering to a communication protocol where each party sequentially sends a message to the next until the last party outputs a valid vertex cover of the whole graph. We are particularly interested in the trade-off between the size of the messages sent and the approximation ratio of the output solution. It is straightforward to see that any constant approximation protocol for MVC requires communicating \(\Omega(n)\) bits. Additionally, there exists a trivial 2-approximation protocol where the parties collectively find a maximal matching of the graph greedily and return the subset of vertices matched. This raises a natural question: \textit{What is the best approximation ratio achievable using optimal communication of \(O(n)\)?} We design a protocol with an approximation ratio of \((2-2^{-k+1}+\epsilon)\) and \(O(n)\) communication for any desirably small constant \(\epsilon>0\), which is strictly better than 2 for any constant number of parties. Moreover, we show that achieving an approximation ratio smaller than \(3/2\) for the two-party case requires \(n^{1 + \Omega(1/\lg\lg n)}\) communication, thereby establishing the tightness of our protocol for two parties.

==> macro.tex <==
\newcommand{\E}[0]{\ensuremath{\mathbb{E}}}


\newcommand{\opt}{\ensuremath{\textsc{opt}}\xspace}
\newcommand{\OPT}{\ensuremath{\textsc{OPT}}\xspace}

\newcommand{\alg}[1]{\ensuremath{\mathsf{PickSubgraph}(#1)}}
\newcommand{\weight}[1]{\ensuremath{w(#1)}}
\newcommand{\gain}[1]{\ensuremath{g#1}}

\newcommand{\Stau}[0]{\ensuremath{\epsilon^2 p}}
\newcommand{\apx}[0]{\ensuremath{\epsilon}}

\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\bra}[1]{\left[#1\right]}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\red}[1]{{\color{red}#1}}

\newcommand{\mvc}[1]{\tau\left(#1 \right)}
\newcommand{\MVC}{\text{MVC}}
\newcommand{\out}{\ensuremath{\Pi}}

\newcommand{\buc}[0]{b}

\newcommand\todos[1]{\textcolor{red}{#1}}
\newtheorem*{theorem*}{\textbf{Theorem \ref{thm:upper-mvc}}}
\newtheorem{question}{Question}

==> open.tex <==
\section{Discussion and Open Problems}

Our work leaves a number of directions for future research. First, while we have essentially settled the one-way communication complexity of deriving a 3/2-approximation for minimum vertex cover in the two-party case, the general multi-party case is open: our upper bound on the approximation ratio for the $k$-party case (using linear communication) is likely not tight, and new techniques are needed to extend the lower bound argument to $k$ parties.

An interesting direction would be to explore whether other lower bound techniques for maximum matching, particularly those by Kapralov \cite{DBLP:conf/soda/Kapralov13, DBLP:journals/corr/abs-2103-11669}, can be adapted to the MVC problem on general graphs. Kapralov's work \cite{DBLP:conf/soda/Kapralov13} established a strict separation between the communication complexity required for achieving a $(1-\varepsilon)$-approximation versus a $(2/3+\varepsilon)$-approximation for maximum bipartite matching in the one-way model. His more recent work \cite{DBLP:journals/corr/abs-2103-11669} provides even stronger lower bounds in random-order streams. If such techniques could be adapted to MVC, they might establish tighter lower bounds for $k > 2$ parties, potentially showing whether our protocol's approximation ratio of $(2 - 2^{-k+1} + \varepsilon)$ is optimal for larger values of $k$ as well.

Second, we believe our approach for developing one-way communication protocols by exploiting connections with stochastic problem variants and providing a framework for $k$ parties is general and is applicable to other graph optimization problems. In particular, developing explicit, polynomial-time protocols that match or approximate our bounds would be a significant step toward practical streaming algorithms.

Finally, we would like to further explore the implications for streaming algorithms for minimum vertex cover. Our work suggests that a standard approach for streaming lower bounds via reduction from the communication model will not help resolve the open problem of whether vertex cover can be approximated better than two by a one-pass streaming algorithm with linear space.

==> utils.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{question}{Question}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{tth}[lemma]{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{conj}[lemma]{Conjecture}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{assumption}[lemma]{Assumption}
\newtheorem{invariant}[lemma]{Invariant}

\newenvironment{LabeledProof}[1]{\noindent{\sl Proof of #1. }}{\qed}

\newenvironment{restate}[1]{\textbf{#1} (restated)\textbf{.}\begin{itshape}}{\end{itshape}\vspace{0.3cm}}

\newcommand{\restatethm}[2]{\noindent \textbf{Theorem~#1} (restated) \textbf{.} {\em #2}}

\newcommand{\restateclaim}[2]{\noindent \textbf{Claim~#1} (restated) \textbf{.} {\em #2}}

\newcommand{\restatelem}[2]{\noindent \textbf{Lemma~#1} (restated) \textbf{.} {\em #2}}





